TANGO: Commonsense Generalization in Predicting Tool Interactions for Mobile Manipulators

Robots assisting us in factories or homes must learn to make use of objects as tools to perform tasks, e.g., a tray for carrying objects. We consider the problem of learning commonsense knowledge of when a tool may be useful and how its use may be composed with other tools to accomplish a high-level task instructed by a human. We introduce a novel neural model, termed TANGO, for predicting task-specific tool interactions, trained using demonstrations from human teachers instructing a virtual robot. TANGO encodes the world state, comprising objects and symbolic relationships between them, using a graph neural network. The model learns to attend over the scene using knowledge of the goal and the action history, finally decoding the symbolic action to execute. Crucially, we address generalization to unseen environments where some known tools are missing, but alternative unseen tools are present. We show that by augmenting the representation of the environment with pre-trained embeddings derived from a knowledge-base, the model can generalize effectively to novel environments. Experimental results show a 60.5-78.9% absolute improvement over the baseline in predicting successful symbolic plans in unseen settings for a simulated mobile manipulator.

==> evaluation-ver-1.3.tex <==
\section{Evaluation Procedure}
%\section{Experiments}\label{sec:experiments}
% Evaluation Data set. 
%\subsection{Evaluation Setup}
% 
% Evaluation corpus table. 

\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textbf{Domain}} & \textbf{Dataset} & \multirow{2}{*}{\textbf{Avg. Plan lengths}} & \textbf{Avg. objects}  & \textbf{Avg. tools} \tabularnewline
     & \textbf{Size} &  & \textbf{interactions/plan} & \textbf{interactions/plan}\tabularnewline
    \hline 
    Home & 3540 & 23.25$\pm$12.65 & 4.12$\pm$1.97 & 0.93$\pm$0.70 \tabularnewline
    %\hline 
    Factory & 3920 & 38.77$\pm$23.17 & 4.38$\pm$1.85 & 1.44$\pm$0.97 \tabularnewline
    \hline 
    \hline 
    \multicolumn{3}{|c|}{\textbf{Sample Objects}} & \multicolumn{2}{c|}{\textbf{Sample goal specifications}}\tabularnewline
    \hline 
    \multicolumn{5}{|c|}{Home}\tabularnewline
    \hline 
    \multicolumn{3}{|c|}{\begin{minipage}[t]{0.39\textwidth} fridge, cupboard, tables, \textbf{tray}, \textbf{book}, paper, bottle, \textbf{box}, fruits, \textbf{stick}, milk carton, \textbf{glue}, \textbf{stool}\footnotemark, \textbf{mop},  dirt\end{minipage}} & \multicolumn{2}{c|}{\begin{minipage}[t]{0.35\textwidth} Place milk in fridge, Place fruits in cupboard, Remove dirt from floor, Stick paper to wall, Illuminate room. \vspace{2pt}\end{minipage}}\tabularnewline
    \hline 
    \multicolumn{5}{|c|}{Factory}\tabularnewline
    \hline 
    \multicolumn{3}{|c|}{\begin{minipage}[t]{0.39\textwidth}
        \textbf{ramp}, crates, \textbf{stick}, \textbf{lift}, cupboard, \textbf{ladder}, \textbf{trolley}, \textbf{brick}, generator, \textbf{gasoline}, screw, nail, \textbf{screwdriver}, wood, water.\end{minipage}} & \multicolumn{2}{c|}{\begin{minipage}[t]{0.35\textwidth} Stack crates, Move tools to workbench, Fix board on wall, Turn on the generator, Assemble and paint parts, Clean spilled water. 
        \end{minipage}}\tabularnewline
    \hline 
    \end{tabular}}
    \setlength{\belowcaptionskip}{-10pt}
    \captionof{table}{\footnotesize Dataset characteristics for Home and Factory domains, plans generated by human instructed robot execution. Objects in bold can be used as tools.
    % Put human here
    %Average plan lengths, number of objects interacted in plan and number of tools used in plans with object and goal sets for Home and Factory domains. Objects in bold can be used as tools.
    }
    \label{tab:dataset}
\end{table}
%\textbf{Corpus. } 
%
We collected plan traces from $\mathrm{12}$ human subjects using  
domain randomization with $\mathrm{10}$ scenes and $8$ semantic goals resulting in 
a corpus of $\mathrm{708}$ and $\mathrm{784}$ plans for the 
home and factory domains. 
%
Data augmentation is performed by perturbing the metric states in the 
human plan trace, performing random replacements of 
scene objects and validating plan feasibility in simulation. 
%
The process results in $\mathrm{3540}$ and $\mathrm{3920}$ plans,  
respectively. 
%for the home and factory domains, respectively. 
%
Table~\ref{tab:dataset} lists data set characteristics. 
%plan diversity,  and shows the 
%variation of actions, total plan simulation time, number of interacted 
%objects and tools with goals in each domain. 
% The process results in $\mathrm{3540}$ and $\mathrm{3920}$ plans for 
% the home and factory domains, respectively. 
%
%Table~\ref{tab:dataset} analyzes the plan diversity and shows the 
%dataset sizes with variation of actions, total plan simulation time, number of interacted 
%objects and tools with goals in each domain. 
%
Variation was observed in tool use for a subject for different 
goals, and within similar goals based on context. 
Further, variation was observed to increase with plan length.
%
%Further, contextual adaptation was observed, for instance, a tray that is closer 
%is more likely to be chosen by a human instructor compared to a box far away. 
%
\footnotetext[1]{Stool/ladder are objects used to represent a tool for raising the height of the robot.}

%
%\textbf{Virtual Environment. }  
%
A physics simulation environment~\cite{coumans2016pybullet} 
was used to generate home and  factory-like environments  
populated with a virtual mobile manipulator (A Universal Robotics (UR5) arm 
mounted on a Clearpath Husky mobile base).
%
The robot is tasked with goals that involve multiple interactions with objects  
derived from standardized data sets \cite{calli2017ycb}. 
%
%We only simulate feasible atomic robot actions and do not encode semantic 
%information about how robot actions can be sequenced for attaining a goal. 
%
A human instructor instructs the robot with a sequence of 
actions required to complete the task. 
%
%The aggregated plans and the environment states form the training data set.  

%\textbf{Test and Generalization Data sets. } 
%  
The evaluation corpus was split as $(75\%:25\%)$ forming the training set and test sets 
to evaluate model accuracy. $10\%$ of training data was used as the validation set for 
hyper-parameter search. 
%
%To assess model accuracy, the the data set corresponding to $9$ scenes 
%as the training set and split data for the remaining scene instance equally 
%forming \emph{validation} and \emph{test} sets. 
%
To assess model generalization to unseen worlds, a data set was 
formed by randomly sampling unseen object locations and object replacement.
%
The following sampling strategies are used: 
(i) \emph{Position}: perturbing and exchanging object positions in a scene.
(ii) \emph{Alternate}: removal of the most frequently used tool in demonstrated plans
evaluating the ability to predict the alternative, next best tool to use.
(iii) \emph{Unseen}: replacing an object with a similar object, which is not present in training.
(iv) \emph{Random}: replacing a tool with random objects unrelated to the task.
(v) \emph{Goal}: replacing objects of training goals with new objects.

%\begin{itemize}
%\item Position: perturbing and exchanging object positions in a scene 
%\item Alternate: removal of the most frequently used tool in demonstrated plans 
%evaluating the ability to predict the alternative, next best tool to use
%\item Unseen: introducing a an object in a scene from a corpus not present in training 
%\item Random: replacing a tool with random objects unrelated to the task
%\item Goal: assess prediction of alternate plans with goals predicated on new objects
%\end{itemize}
%\textbf{Metrics and Baseline. }  
%
The following metrics were used for model evaluation:  
(i) \emph{Action prediction accuracy}: the fraction of tool interactions predicted by the model 
which matched the human demonstrated action $a_t$ for a given state $s_t$, and 
(ii) \emph{Plan execution accuracy}: the fraction of estimated plans that are successful, i.e., can be executed by the 
robot in simulation and attain the intended goal (in max. $50$ steps).    
%\begin{itemize} 
%\item \emph{Action Prediction Accuracy}: fraction of tool interactions predicted by the model 
%which matched the human demonstrated action $a^j_t$ for a given state $s^j_t$, and 
%\item \emph{Plan Execution Accuracy}: fraction of estimated plans that are successful, i.e., can be executed by the 
%robot in simulation and attain the intended goal (upto $T=50$ length plans).  
%\end{itemize} 
%
%
The state of the art \emph{ResActGraph} model \cite{liao2019synthesizing} 
augmented with $\mathrm{FastText}$ embeddings \cite{mikolov2018advances} as $\mathcal{C}(\cdot)$ function, served as the 
baseline model for all experiments. 
%
%For a fair comparison, the model was augmented with word embeddings following 
%\cite{sunderhauf2019keys}. 
%
The data set, code and experimental details are submitted as part of supplementary material.

% Results
\section{Results}
%
% Main Model Accuracy Table
\begin{table*}
    \centering
    \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{|c !{\vrule width1pt}c|c !{\vrule width1pt}c|c !{\vrule width1pt}c|c|c|c|c|c|c|}
    \hline 
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c !{\vrule width0.8pt}}{\textbf{Action Prediction}} & \multicolumn{2}{c !{\vrule width0.8pt}}{\textbf{Plan Execution}} & \multicolumn{7}{c|}{\textbf{Generalization Plan Execution Accuracy}}\tabularnewline
    \cline{2-12} 
     & Home & Factory & Home & Factory & Home & Factory & Position & Alternate & Unseen & Robust & Goal\tabularnewline
    \hline
    \hline
    Baseline (ResActGraph) & 27.67 & 45.81 & 26.15 & 0.00 & 12.38 & 0.00 & 0.00 & 0.00 & 0.00 & 25.10 & 9.12\tabularnewline
    \hline
    Affordance Only & 46.22 & 52.71 & 52.12 & 20.39 & 44.10 & 4.82 & 17.84 & 47.33 & 29.31 & 29.57 & 34.85\tabularnewline
    \hline
    DQN  & - & - & 24.82 & 17.77 & 15.26 & 2.23 & 0.00 & 0.00 & 12.75 & 9.67 & 4.21\tabularnewline
    \hline 
    \modelname & 59.43 & 60.22 & 92.31 & 71.42 & \textbf{91.30} & \textbf{60.49} & \textbf{93.44} & \textbf{77.47} & \textbf{81.60} & 59.68 & \textbf{59.41}\tabularnewline
    \hline \hline
    \multicolumn{12}{|c|}{Ablation}\tabularnewline
    \hline \hline
    - GGCN (World Representation) & 59.43 & 60.59 & 84.61 & 27.27 & 78.02 & 38.70 & 70.42 & 58.79 & 60.00 & 56.35 & 38.64\tabularnewline
    \hline 
    - Metric (World Representation) & 58.8 & 60.84 & 84.61 & 62.34 & 72.42 & 51.83 & 59.68 & 67.19 & 60.79 & \textbf{84.47} & 21.70\tabularnewline
    \hline 
    - Goal-Conditioned Attn & 53.14 & 60.35 & 53.85 & 11.69 & 37.02 & 8.80 & 35.33 & 15.05 & 32.14 & 41.67 & 6.51\tabularnewline
    \hline 
    - Temporal Action History & 45.91 & 49.94 & 24.61 & 0.00 & 8.55 & 0.00 & 0.00 & 0.00 & 0.00 & 30.56 & 1.15\tabularnewline
    \hline 
    - ConceptNet & \textbf{63.52} & 60.35 & 89.23 & 57.14 & 81.86 & 56.97 & 82.33 & 68.61 & 74.57 & 65.73 & 47.92\tabularnewline
    \hline 
    - Factored Likelihood & 61.32 & \textbf{61.34} & \textbf{95.38} & \textbf{85.71} & 34.22 & 43.44 & 90.50 & 14.82 & 30.65 & 64.67 & 53.26\tabularnewline
    \hline 
    % - Constraints & 57.23 & 57.74 & 64.62 & 37.66 & 62.98 & 41.95 & 84.95 & 45.39 & 39.99 & 36.11 & 84.85\tabularnewline
    % \hline 
    % - Auto-regression & 56.60 & 60.22 & 69.23 & 50.65 & 73.75 & 53.32 & 71.24 & 66.43 & 61.27 & 70.51 & 34.66\tabularnewline
    % \hline 
    \end{tabular}}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{\footnotesize{A comparison of \emph{Action prediction} and \emph{Plan execution} accuracies for the baseline, the proposed \modelname model, and ablations. Results are presented for test and generalization data sets (under five sampling strategies) derived from the home and factory domains. 
     %\textit{Accuracy Prediction} is the percentage of predicted actions matching the human input on the Test set. \textit{Plan Execution} is the percentage of plans successfully executed in the Test set. \textit{Generalization Plan Accuracy} is the percentage of plans successfully executed in the  set.
    }}
    \label{tab:ablation}
\end{table*}


% Model Accuracy
\subsection{Model Accuracy and Generalization}

\subsubsection{Comparison with ResActGraph}
%\textbf{Model accuracy. }
%
\modelname{} demonstrates a 14-23\% increase in 
\emph{action prediction accuracy} compared to the baseline 
and demonstrates accurate predictions in novel contexts with 
different object placements and positions. 
%
See Table~\ref{tab:ablation}. 
%
The model shows a 66-71\% increase in 
the ability to synthesize a plan of tool interactions that  
reach the intended goal. 
%
% Further, the fraction of times when the model is unable to reach the goal 
% (in up to $50$ steps) is low, see Figure~\ref{fig:errors}. 

%\textbf{Model generalization. }  
%
We assess whether the model can perform common sense 
generalization  in worlds with new 
objects unseen in training. 
%
Table~\ref{tab:ablation} illustrates that the interaction sequences predicted 
by \modelname lead to a $60-79\%$ increase in plan execution accuracy on Generalization Test set. 
%
The model is able to infer the utility of new objects for a given goal. 
%
For example, in home domain, if the \emph{stool} is not present in the scene, 
the model uses a \emph{stick} instead to fetch far-away objects. 
%
Further, in the factory domain, if \emph{coal} is removed from 
the scene, the model uses \emph{gasoline} 
to power the generator. 
%
Implicitly, the model learns a context for a goal, associating 
objects with tasks. Further, the adoption of distributional semantics 
via $\mathrm{ConceptNet}$ embeddings enable generalization to new objects 
that share semantic properties.

\subsubsection{Comparison with Direct Affordance Prediction}

We compared \modelname with a simple approach of learning object affordances~\cite{hermans2011affordance}. 
% For this, we created an affordance-only neural model that uses pre-trained ConceptNet embeddings, along with the scene graph, metric properties, goal and action history to predict the next action. This model excludes graph convolutions, and spatial attention components of \modelname.
We adapted \modelname to create an affordance-only model by excluding graph convolution and spatial attention components.
The model performed 40-50\% and 47-56\% worse than TANGO on regular and generalization test sets (Table~\ref{tab:ablation}).
%
We conducted generalization tests in environments with unseen objects,
by substituting objects in the demonstrations using a similarity-metric from ConceptNet relations. 
The performance of such a rule based approach was much lower with 91-56\% drop in accuracies on two domains. 
Thus, a simple affordance model is insufficient for our task as it ignores the 
temporal associations between tool use.

%

%\textbf{Plan length comparisons. } 
% Figure~\ref{fig:planlen} compares the lengths of robot plans 
% predicted by the learned model with the set of human demonstrated plans. 
% %
% We observe that, on average, the predicted plan lengths are 
% close to the human demonstrated ones. 
% %
% Analyzing the cases where predicted plans are longer, we find that \modelname  prediction of spurious actions, 
% e.g., in the factory domain, the robot fetches and places a ramp 
% even when all the items to be moved are on the same level. 
% %
% In 12\% of the cases, the model utilizes a more appropriate tool 
% to reach the goal state faster than a human. 


% %% Robustness
% \begin{wrapfigure}[16]{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/robust.pdf}
%     \caption{\footnotesize{Plan adaptation in presence of execution errors and stochasticity.}} 
%     \label{fig:robust}
% \end{wrapfigure}
%% Plan Execution Film Strip: Generalization
\subsection{Experiments on a simulated robot}
%\textbf{Demonstration on a simulated robot. }  
%
Figure \ref{fig:plans} demonstrates the robot using the learned model to synthesize 
a plan for a declarative goal. 
%
Here, if the goal is to transport fruits and human demonstrates usage of \emph{tray} and the model never sees \emph{box} while training. \modelname uses \emph{box} in a scene where tray is absent, showing that it is able to predict semantically similar tools for task completion. Similarly, for the goal of fixing a board on the wall, if humans use \emph{screws} the agent uses \emph{nails} and \emph{hammer} when screws are absent from the scene. 
%
Figure~\ref{fig:robust} shows the robustness to unexpected errors and stochasticity. 
%
% Since, in the domain complex errors can occur during execution. 
% The learned model predicts the use appropriate tools to mitigate the 
% effect of the errors leading to robust plan execution. 
%
For the goal of "fetch carton", where the milk carton is on an elevated platform, the model predicts the uses a stool to elevate itself. 
The carton falls due to errors during action execution. 
Detecting this, the robot infers that the stool is no longer required and directly fetches the carton. 
%
\begin{figure}[!t]
    \centering
    \begin{minipage}{\columnwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/plan_synthesis.pdf}
        \caption{
        \footnotesize{
        A simulated robot manipulator uses \modelname to synthesize tool interactions in 
        novel contexts with unseen objects. 
        %\text{Plan Synthesis.} Two output plans by \modelname in novel settings of home and factory domains.}
        }}
        \label{fig:plans}
    \end{minipage}\ 
    % \begin{minipage}{.495\textwidth}
    %     \centering
    %     \includegraphics[width=0.49\linewidth]{figures/planlen/legend.pdf}\\
    %     \begin{subfigure}{0.49\linewidth}
    %         \centering
    %         \includegraphics[width=\linewidth]{figures/planlen/test_home.pdf}
    %         \caption{Home domain}
    %         \label{fig:len_home}
    %     \end{subfigure}
    %     \begin{subfigure}{0.49\linewidth}
    %         \centering
    %         \includegraphics[width=\linewidth]{figures/planlen/test_factory.pdf}
    %         \caption{Factory Domain}
    %         \label{fig:len_factory}
    %     \end{subfigure}
    %     \caption{\footnotesize{Avg. length of plans inferred by  
    %     \modelname  (green) and demonstrated by human subjects (blue).}} 
    %     \label{fig:planlen}
    % \end{minipage}
\end{figure}


% \begin{wrapfigure}[12]{r}{0.5\columnwidth}
%         \centering
%         \includegraphics[width=0.95\linewidth]{figures/planlen_scatter.pdf}
%         \caption{\footnotesize{Scatter plot comparing plan lengths of model and human demonstrations (Test Set).}} 
%         \label{fig:planlen}
% \end{wrapfigure}

% \begin{figure}
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline 
%     \multicolumn{5}{|c|}{Home: Place fruits in cupboard generalization test case (\emph{tray} unavailable)}\tabularnewline
%     \hline 
%     \includegraphics[width=0.195\textwidth]{figures/home_strip2/0} & \includegraphics[width=0.195\textwidth]{figures/home_strip2/29} & \includegraphics[width=0.195\textwidth]{figures/home_strip2/204} & \includegraphics[width=0.195\textwidth]{figures/home_strip2/216} & \includegraphics[width=0.195\textwidth]{figures/home_strip2/243}\tabularnewline
%     \hline 
%     0: Start state & 1: Open cupboard & 2: Place fruits in box & 3: Pick box & 4: Place box in cupboard\tabularnewline
%     \hline 
%     \multicolumn{5}{|c|}{Factory: Fix board on wall generalization test case (\emph{screws} unavailable)}\tabularnewline
%     \hline 
%     \includegraphics[width=0.195\textwidth]{figures/factory_strip/0} & \includegraphics[width=0.195\textwidth]{figures/factory_strip/21} & \includegraphics[width=0.195\textwidth]{figures/factory_strip/80} & \includegraphics[width=0.195\textwidth]{figures/factory_strip/177} & \includegraphics[width=0.195\textwidth]{figures/factory_strip/214}\tabularnewline
%     \hline 
%     0: Start state & 1: Place ramp & 2: Pick Board & 3: Place board on wall & 4: Hammer nail on board\tabularnewline
%     \hline 
%     \end{tabular}
%     }
%     \caption{
%     \footnotesize{\text{Plan Synthesis.} Two output plans by \modelname in novel settings of home and factory domains.}
%     }
%     \label{fig:plans}
% \end{figure}

% % Plan length comparisons. 
% \begin{wrapfigure}[13]{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.49\linewidth]{figures/planlen/legend.pdf}\\
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/planlen/test_home.pdf}
%         \caption{Home domain}
%         \label{fig:len_home}
%     \end{subfigure}
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/planlen/test_factory.pdf}
%         \caption{Factory Domain}
%         \label{fig:len_factory}
%     \end{subfigure}
%     \caption{\footnotesize{Avg. length of plans inferred by  
%     \modelname  (green) and demonstrated by human subjects (blue).}} 
% %    for Home (left) and Factory (right) domains. }}
%     \label{fig:planlen}
% \end{wrapfigure}

\begin{figure}
        \centering
        \setlength{\belowcaptionskip}{-10pt}
        \includegraphics[width=0.5\textwidth]{figures/robust.pdf}
        \caption{\footnotesize{Interleaved action prediction and 
        execution enables adaptation in case of unexpected errors during action execution. }} 
        \label{fig:robust}
\end{figure}


% Ablation Analysis
\subsection{Ablation Analysis} 
%\textbf{Ablation analysis. }   
Table~\ref{tab:ablation} (ablation study) studies 
the effect of removal of each component on the TANGO model.
 % 
% Figure~\ref{fig:errors} analyses the type of prediction errors. 
 %
For a fair comparison the model capacities were kept constant during the ablation experiments.  
%
%The graph-structured representation (\emph{GGCN}) models the 
%relational structure of the domain. 
%
The GGCN component, which models the relational structure, contributes towards learning the need to move close to a tool before interacting with it, 
using a ramp to negotiate an elevation or using a stick to fetch 
object outside reach. 
%
Inclusion of metric properties (\emph{Metric}) such as 
physical volume and axes extent allows the model to infer 
tool interaction based on relative sizes. 
%
E.g., predicting that \emph{fruits} can be transported  
using a \emph{tray} but larger \emph{cartons} require a \emph{box} to be carried. 
%
The inclusion of ConceptNet embeddings is crucial for predicting 
interactions with unseen tools. 
%
The dense representation of object types allows generalization 
based on shared semantic attributes. 
%
The baseline with $\mathrm{FastText}$
\cite{mikolov2018advances} word embeddings shows poorer generalization (6.5\% decrease). 
%
This is attributed to the fact that $\mathrm{FastText}$ embeddings model 
word affinity as expressed in language only. 
%
On the other hand, 
$\mathrm{ConceptNet}$ embedding space additionally models relational affinity 
between objects as maintained in the knowledge-base. 
%
%as they do not model semantic relations \emph{between} object types. 
%On the other hand, \emph{ConceptNet} embeddings 
%explicitly model semantic relationships.  

%
The removal of the Goal-Conditioned Attention component leads to 
a significant reduction of ($\approx 50$ points) in plan execution accuracy on Generalization Test set, 
particularly in scenes with a large number of objects. 
%
The ability to attend to goal relevant objects allows learning 
of a task relevant context of a smaller number of objects, particularly 
in workspaces with a large number of objects. 
%
Finally, the Action History component models the agent's state 
during the plan execution. 
%
The component learns correlation between action types 
and learns that certain plan fragments are very common 
e.g., moving to a door, opening it and moving outside. 
%
Removing this component leads to errors such as the robot 
trying to pick an object inside an enclosure without opening the lid. 

\subsection{Comparison with a vanilla RL model}

We also compared the model with a vanilla RL-model, Deep Q-Learning (DQN) for this task~\cite{bae2019multi}. Due to the size of the problem (1000 actions), long plans, sparse and delayed rewards (no reward until goal achievement), we were unable to scale RL to our problems, and achieved less than 20\% policy accuracy after a week of training. In contrast, our reported results are obtained after training on imitation learning data for 12-18 hours.

% \subsection{Other Insights}
%\textbf{Comparison with vanilla affordance prediction.}


%\textbf{Comparison with RL.}


% \begin{table}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|c !{\vrule width1pt}c|c !{\vrule width1pt}c|c|c|c|c|c|c|}
%     \hline 
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c !{\vrule width0.8pt}}{\textbf{Plan Execution}} & \multicolumn{7}{c|}{\textbf{Generalization Plan Execution Accuracy}}\tabularnewline
%     \cline{2-10} 
%      & Home & Factory & Home & Factory & Position & Alternate & Unseen & Robust & Goal\tabularnewline
%     \hline
%     \hline
%     DQN  & 24.82 & 17.77 & 15.26 & 2.23 & 0.00 & 0.00 & 12.75 & 9.67 & 4.21\tabularnewline
%     \hline 
%     \modelname & \textbf{92.31} & \textbf{71.42} & \textbf{91.30} & \textbf{60.49} & \textbf{93.44} & \textbf{77.47} & \textbf{81.60} & \textbf{59.68} & \textbf{59.41}\tabularnewline
%     \hline 
%     \end{tabular}}
%     \caption{\footnotesize{Comparison with a simple RL model.}}
%     \label{tab:rl}
% \end{table}

%
% \textbf{Limitations and future work. }
% %
% Figure~\ref{fig:test} examines model accuracy in relation to plan length.
% %
% The plan execution accuracy decreases by 20\% on Test and 
% 30\% on Generalization Test sets from the home domain to 
% the factory domain. 
% %
% This is attributed to longer interaction sequences in larger and 
% more complex worlds in the factory domain. 
% %
% \begin{figure}[!t]
%     \centering
%     \begin{minipage}{.335\columnwidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{figures/perflen2/test.pdf}
%         \captionof{figure}{\footnotesize{Execution accuracy of inferred plans with plan length.}}
%         \label{fig:test}
%     \end{minipage}\ \ 
%     \begin{minipage}{.64\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/errors.pdf}
%       \captionof{figure}{\footnotesize{Analysis of fractional errors during plan execution using the learned model.}}
%         \label{fig:errors}
%     \end{minipage}
%     % \captionof{figure}{\footnotesize{Plan execution accuracy on Test set reduces as goal/environment becomes more complex and longer plans are required to reach to the goal state.}}
%     \label{fig:perflen}
% \end{figure}
% %
% Learning the temporal pre-conditions for actions such 
% as the robot's gripper needs to be free before manipulating an object 
% are challenging, Figure~\ref{fig:errors}. 
% %
% There is scope for improvement by explicitly modeling causal structure following \cite{nair2019causal}. 
% %
% The proposed model ignores 
% the metric feasibility of sequential actions assuming that the human provides feasible plans 
% hence merits future investigation into integration with a  
% \emph{task and motion planner}  
% with (near) optimality \cite{driess2020deep, vega2020asymptotically} 
% or verification \cite{fainekos2005temporal} guarantees for plans. 
%
%Future work will address experiments on a physical platform and 
%extend the model to partially-known and uncertain worlds. 

